Deep Plug-and-Play Proximal Distance Algorithm for Robust Principal Component Analysis

Robust Principal Component Analysis (RPCA) is essential in signal processing, with applications in hyperspectral imaging, face recognition, and video background modeling. Traditional RPCA methods often suffer from insufficient utilization of data priors and struggle to capture complex image structures. Conversely, advanced deep denoisers like DnCNN, FFDNet, and DRUNet excel at leveraging image data priors but lack physical model constraints and demonstrate poor robustness against structured noise in RPCA tasks. This paper proposes a novel Plug-and-Play (PnP) method for multi-channel RPCA, integrating both the physical generative model and cutting-edge deep priors. Extensive experiments on RGB and hyperspectral datasets show that PnP-PDA achieves better quantitative performance than conventional RPCA methods and state-of-the-art methods, including deep denoisers and tensor RPCA approaches, while preserving visual details.

==> sym_marco.tex <==
%make sure to keep this for convenience later
\newcommand\bw{\ensuremath{{\bm w}}}
\newcommand\bW{\ensuremath{{\bm W}}}
\newcommand\cW{\ensuremath{\bm{\mathcal{W}}}}
\newcommand\bbw{\ensuremath{{\bar{\bm w}}}}
\newcommand\bq{\ensuremath{{\bm q}}}
\newcommand\bx{\ensuremath{{\bm x}}}
\newcommand\by{\ensuremath{{\bm y}}}
\newcommand\bG{\ensuremath{{\bm G}}}
\newcommand\bh{\ensuremath{{\bm h}}}
\newcommand\bH{\ensuremath{{\bm H}}}
\newcommand\cH{\ensuremath{\bm{\mathcal{H}}}}
\newcommand\bbh{\ensuremath{\bar{\bm h}}}
\newcommand\hbh{\ensuremath{\hat{\bm h}}}
\newcommand\be{\ensuremath{{\bm e}}}
\newcommand\bz{\ensuremath{{\bm z}}}
\newcommand\bp{\ensuremath{{\bm p}}}
\newcommand\bP{\ensuremath{{\bm P}}}
\newcommand\bR{\ensuremath{{\bm R}}}
\newcommand\bT{\ensuremath{{\bm T}}}
\newcommand\bX{\ensuremath{{\bm X}}}
\newcommand\bZ{\ensuremath{{\bm Z}}}
\newcommand\cZ{\ensuremath{\bm{\mathcal{Z}}}}
\newcommand\bC{\ensuremath{{\bm C}}}
\newcommand\bc{\ensuremath{{\bm c}}}
\newcommand\ba{\ensuremath{{\bm a}}}
\newcommand\bba{\ensuremath{\bar{\bm a}}}
\newcommand\bA{\ensuremath{{\bm A}}}
\newcommand\bbA{\ensuremath{\bar{\bm A}}}
\newcommand\bb{\ensuremath{{\bm b}}}
\newcommand\bg{\ensuremath{{\bm g}}}
\newcommand\bB{\ensuremath{{\bm B}}}
\newcommand\blam{\ensuremath{{\bm \lambda}}}
\newcommand\bmu{\ensuremath{{\bm \mu}}}
\newcommand\balp{\ensuremath{{\bm \alpha}}}
\newcommand\bbeta{\ensuremath{{\bm \beta}}}
\newcommand\bXi{\ensuremath{{\bm \Xi}}}
\newcommand\bPi{\ensuremath{{\bm \Pi}}}
\newcommand\bbPi{\ensuremath{\bar{\bm \Pi}}}
\newcommand\bF{\ensuremath{{\bm F}}}
\newcommand\bbF{\ensuremath{\bar{\bm F}}}
\newcommand\bd{\ensuremath{{\bm d}}}
\newcommand\bD{\ensuremath{{\bm D}}}
\newcommand\bN{\ensuremath{{\bm N}}}
\newcommand\bu{\ensuremath{{\bm u}}}
\newcommand\bnu{\ensuremath{{\bm \nu}}}
\newcommand\bv{\ensuremath{{\bm v}}}
\newcommand\bSig{\ensuremath{{\bm \Sigma}}}
\newcommand\bsig{\ensuremath{{\bm \sigma}}}
\newcommand\beeta{\ensuremath{{\bm \eta}}}
\newcommand\bphi{\ensuremath{{\bm \phi}}}
\newcommand\bPhi{\ensuremath{{\bm \Phi}}}
\newcommand\bPsi{\ensuremath{{\bm \Psi}}}
\newcommand\btheta{\ensuremath{{\bm \theta}}}
\newcommand\tbtheta{\ensuremath{\tilde{\bm \theta}}}
\newcommand\bvartheta{\ensuremath{{\bm \vartheta}}}
\newcommand\bTheta{\ensuremath{{\bm \Theta}}}
\newcommand\bomega{\ensuremath{{\bm \omega}}}
\newcommand\bxi{\ensuremath{{\bm \xi}}}
\newcommand\bzeta{\ensuremath{{\bm \zeta}}}
\newcommand\bpi{\ensuremath{{\bm \pi}}}

\newcommand\bYh{\ensuremath{{\bm Y}_{\rm H}}}
\newcommand\bYm{\ensuremath{{\bm Y}_{\rm M}}}
\newcommand\byh{\ensuremath{{\bm y}_{\rm H}}}
\newcommand\bym{\ensuremath{{\bm y}_{\rm M}}}
\newcommand\bAm{\ensuremath{{\bm A}_{\rm M}}}
\newcommand\bDh{\ensuremath{{\bm D}_{\rm H}}}
\newcommand\bDm{\ensuremath{{\bm D}_{\rm M}}}
\newcommand\bDx{\ensuremath{{\bm D}_{\rm X}}}
\newcommand\bVh{\ensuremath{{\bm V}_{\rm H}}}
\newcommand\bVm{\ensuremath{{\bm V}_{\rm M}}}
\newcommand\Lh{\ensuremath{L_{\rm H}}}
\newcommand\Mm{\ensuremath{M_{\rm M}}}


\newcommand\bY{\ensuremath{{\bm Y}}}
\newcommand\bV{\ensuremath{{\bm V}}}
\newcommand\bU{\ensuremath{{\bm U}}}
\newcommand\bs{\ensuremath{{\bm s}}}
\newcommand\bS{\ensuremath{{\bm S}}}
\newcommand\bE{\ensuremath{{\bm E}}}

\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Sbb}{\mathbb{S}}

\newcommand{\setA}{\mathcal{A}}
\newcommand{\setB}{\mathcal{B}}
\newcommand{\setD}{\mathcal{D}}
\newcommand{\setH}{\mathcal{H}}
\newcommand{\setX}{\mathcal{X}}
\newcommand{\setR}{\mathcal{R}}
\newcommand{\setU}{\mathcal{U}}
\newcommand{\setV}{\mathcal{V}}
\newcommand{\setW}{\mathcal{W}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setC}{\mathcal{C}}
\newcommand{\setN}{\mathcal{N}}
\newcommand{\setL}{\mathcal{L}}
\newcommand{\setP}{\mathcal{P}}
\newcommand{\setQ}{\mathcal{Q}}
\newcommand{\setY}{\mathcal{Y}}
\newcommand{\setK}{\mathcal{K}}

\newcommand{\N}{\mathcal{N}}
\newcommand{\CN}{\mathcal{CN}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\jj}{\mathfrak{j}}
\newcommand{\dec}{\mathrm{dec}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\diag}{\mathrm{diag}}

\newcommand\bQ{\ensuremath{{\bm Q}}}
\newcommand\bLam{\ensuremath{{\bm \Lambda}}}
\newcommand\br{\ensuremath{{\bm r}}}

\newcommand\Ree{\ensuremath{{\rm Re}}}
\newcommand\Imm{\ensuremath{{\rm Im}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\bzero}{{\bm 0}}
\newcommand{\bone}{{\bm 1}}
\newcommand{\bI}{{\bm I}}
\newcommand*{\LargerCdot}{\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}
\newcommand\vvec{\ensuremath{{\rm vec}}}
\newcommand\mmat{\ensuremath{{\rm mat}}}
\newcommand\bigO{\ensuremath{{\mathcal{O}}}}

\newcommand{\lammax}{\lambda_{\rm max}}
\newcommand{\lammin}{\lambda_{\rm min}}
\newcommand{\betamaxi}{\beta^{\sf max}_i}
\newcommand{\betamini}{\beta^{\sf min}_i}
%\newcommand{\hbetamini}{\hat{\beta}^{\sf min}_i}
\newcommand{\hbetamini}{{\delta_i}}
%\newcommand\hbetamin[1]{\hat{\beta}^{\sf min}_{#1}}
\newcommand\hbetamin[1]{{\delta_{#1}}}
\newcommand{\hbetainiti}{\hat{\beta}^{\sf init}_i}

%\newcommand{\hbetai}{{\green \hat{\beta}_i(\bx_{-i})}}
\newcommand{\hbetai}{{\hat{\beta}_i}}
\newcommand{\hRi}{{\hat{\bR}_i}}

\newcommand{\aalp}{{\alpha_i}}
\newcommand\aaalp[1]{{\alpha_{#1}}}
\newcommand{\setI}{\mathcal{I}}

\newcommand\indfn[1]{{{\mathbbm 1}_{#1}}}
%\newcommand\indfn{\ensuremath{{\mathbbm 1}}}
%\newcommand\prox{\ensuremath{{\sf prox}}}
\newcommand\prox{\ensuremath{{\rm prox}}}
\newcommand\Prox{\ensuremath{{\rm Prox}}}
\newcommand\LO{\ensuremath{{\sf LO}}}

\newcommand\update{\ensuremath{{\sf UD}}}
\newcommand\bxex{\ensuremath{{\bm x}_{\rm ex}}}
\newcommand\bxkil{\bm x^{k,i,\ell}}
\newcommand\bxki[1]{\bm x^{k,i,#1}}
\newcommand\bxk[2]{\bm x^{k,#1,#2}}
\newcommand\dF[1]{\Delta_{#1}}
\newcommand\dx[1]{e_{#1}}
\newcommand\tdx[1]{\tilde{e}_{#1}}

\newcommand\A[1]{{\sf A#1)}}

\newcommand\dom{\ensuremath{{\rm dom}\,}}
\newcommand\sspan{\ensuremath{{\rm span}}}
\newcommand\aff{\ensuremath{{\rm aff}}}
\newcommand\conv{\ensuremath{{\rm conv}}}
\newcommand\cone{\ensuremath{{\rm cone}}}
\newcommand\cl{\ensuremath{{\rm cl}}}
\newcommand\inte{\ensuremath{{\rm int}}}
\newcommand\bnd{\ensuremath{{\rm bd}}}
\newcommand\bconv{\ensuremath{\overline{\rm conv}}}
\newcommand\var{\ensuremath{{\rm var}}}
\newcommand\cov{\ensuremath{{\rm Cov}}}
\newcommand\svol{\ensuremath{{\rm vol}}}
\newcommand\TVar{\ensuremath{{\rm tvar}}}
\newcommand\tr{\ensuremath{{\rm tr}}}
\newcommand\her{\ensuremath{{\sf H}}}
\newcommand\Ind{\ensuremath{{\mathbbm I}}}   

